Assessing the Viability of Synthetic Physical Copy Detection Patterns on Different Imaging Systems

This paper explores the potential of synthetic physical Copy Detection Patterns (CDP) to improve the robustness of anti-counterfeiting systems. By leveraging synthetic physical CDP, we aim at enhancing security and cost-effectiveness across various real-world applications. Our research demonstrates that synthetic CDP offer substantial improvements in authentication accuracy compared to one based on traditional digital templates. We conducted extensive tests using both a scanner and a diverse range of mobile phones, validating our approach through ROC analysis. The results indicate that synthetic CDP can reliably differentiate between original and fake samples, making this approach a viable solution for real-world applications, though requires an additional research to make this technology scalable across a variety of imaging devices.

==> sections/01_introduction_old.tex <==
\section{Introduction}

Copy Detection Patterns (CDP) have emerged as a promising anti-counterfeiting technology, gaining traction due to their cost-effectiveness, scalability, and ease of integration across various industries. These patterns can be applied to a wide range of materials and products, including packaging, security labels, pharmaceutical products, currency, and identification documents. Their effectiveness stems from their inherent resistance to replication, machine verifiability, and versatility. Recent advancements have further enhanced their applicability, allowing for product verification directly by end customers using mobile phone technologies. Despite these advantages, recent studies have revealed potential vulnerabilities in CDP, such as susceptibility to forgery attacks and variability due to manufacturing parameters. These findings highlight the need for ongoing R\&D to tackle security challenges and strengthen CDP's robustness in crucial applications.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/lifecycle.png}
    \caption{The diagram demonstrating the real-world CDP lifecycle which includes the authentication of probe $\y$, the possible attack scenario (red dashed line) yielding fake $\f$ and the proposed defensive strategies (green dashed line).}
    \label{fig:lifecycle}
    \vspace{-7mm}
\end{figure}

Sophisticated machine learning attacks have been shown to be highly effective against CDP, significantly compromising its security. These attacks leverage advanced algorithms to create high-quality fake CDP $\f$ that can bypass existing authentication methods. As a result, the robustness of CDP is called into question, particularly in critical sectors such as pharmaceuticals. The most efficient countermeasure identified to date is the use of physical CDP $\x$, which offers superior protection against such sophisticated attacks. However, for its authentication, it is required to have the enrollment CDP $\xe$, which negates its main advantage, cost-effectiveness.

To balance cost and authentication accuracy, in this study, we address and endorse the use of synthetic physical CDP $\xhat$. This approach serves as a viable trade-off, mitigating the high acquisition costs of $\xe$ while enhancing the low authentication accuracy often associated with digital template $\t$. Synthetic $\xhat$ combines the benefits of both physical and digital systems, providing a more secure and economical solution. Our study evaluates the effectiveness of this approach using both scanners and mobile phones, aiming to provide a comprehensive understanding of its practical application.

The study involves extensive testing to demonstrate scanner-derived statistics as the baseline. Scanners, known for their high precision and consistency, provide reliable data for evaluating the performance of CDP but are not considered as the real-world example of the verification device. Thus, we test a wide range of mobile devices, from the iPhone XS (released in 2018), to the iPhone 15 Pro Max (2023). This diverse range allows us to assess the robustness of $\xhat$ across different imaging systems, which vary significantly in terms of optical capabilities, sensor size, focal length, and field of view (FOV). By including a broad spectrum of devices in our study, we aim to ensure that $\xhat$ can perform reliably under various conditions.

The goal of this study is threefold. Firstly, we aim to highlight the necessity of synthetic CDP $\xhat$, as they significantly improve performance compared to methods based on digital template CDP $\t$. Secondly, we claim that for certain applications, the use of high-end mobile phones is currently sufficient for regular authentication with respect to $\t$ in contrast to devices with a lower effective resolution. However, this situation may change in the future as technology and counterfeiting techniques evolve. Thirdly, we do not intend to demonstrate the best synthetic CDP in this study. Instead, we employ a simplistic methodology to address current issues and promote the adoption of $\xhat$ over $\t$ or $\xe$ as a reference for similarity assessment. As for the similarity assessment, we continue to rely on Pearson correlation index $\fpcorr$ and SSIM $\fssim$ to stay well-aligned with previous studies on CDP.

In conclusion, the use of synthetic physical CDP presents a promising solution to the vulnerabilities identified in traditional CDP systems. By leveraging both physical and digital advantages, this approach can offer enhanced security and cost-effectiveness. Our comprehensive study, involving both scanner and mobile phone evaluations, aims to validate this solution and provide a robust framework for its implementation across various industries. The findings will contribute to the ongoing development of more secure and efficient anti-counterfeiting technologies, ensuring the protection of critical products and documents against sophisticated counterfeiting threats. As the most reasonable takeaway of this study we plan to assess the viability of synthetic CDP when used across different imaging systems simultaneously. Specifically, we will explore how synthetic CDP estimators trained on one mobile phone model perform in verifying probes from different imaging systems.

==> sections/01_lifecycle.tex <==
\section{Variations of Copy Detection Patterns (CDP) and Their Roles in Authentication}

This chapter provides an in-depth explanation of the various forms of Copy Detection Patterns (CDP) and their roles within our proposed authentication system. The different types of CDP are visualized in the figure, highlighting the life cycle and application of each variant to combat counterfeiting and ensure robust authentication.

\subsection{Digital Template (\t)}
The digital template, denoted as \t, is the initial digital form of a CDP. This template serves as the basis for generating the physical CDPs and is typically produced using an industrial printer denoted \( P_E \).

\subsection{Physical Original CDP (\x)}
The physical original CDP, denoted as \x, is created by printing the digital template \t using the industrial printer \( P_E \). This physical CDP is then distributed to the public domain and can be authenticated by comparing acquired images to a reference.

\subsection{Estimation of Sophisticated Attack (\th)}
In scenarios where an attacker uses sophisticated methods, such as machine learning, to estimate the original digital template, the result is denoted as \th. This estimated template is then reprinted using a different printer, \( P_A \), leading to a fake CDP.

\subsection{Fake CDP (\f)}
The fake CDP, denoted as \f, is produced by reprinting the estimated digital template \th using the attacker printer \( P_A \). This fake CDP is distributed in the same public domain as the original CDP, complicating the authentication process.

\subsection{Synthetic Original CDP (\xh)}
The synthetic original CDP, denoted as \xh, is created by transforming the digital template \t into a synthetic physical template. This synthetic CDP can be generated on-the-fly for any unseen template, offering flexibility and robustness in the authentication process.

\subsection{Enrolled Original Physical CDP (\xe)}
The enrolled original physical CDP, denoted as \xe, is a physical CDP captured and stored at the stage of production before public distribution. This enrolled CDP serves as a reference for authentication, using the unique physical characteristics of the original CDP.

\subsection{Reference CDP (\r)}
The reference CDP, denoted as \r, can be either the digital template \t, the synthetic original CDP \xh, or the enrolled original physical CDP \xe. This reference is used in the similarity assessment to authenticate incoming probes.

\subsection{Probe (\y)}
The probe, denoted \y, represents the CDP being authenticated. It can be either an original or fake CDP, and its origin is unknown at the time of verification. The probe \y is compared to the reference \r using similarity metrics.

\subsection{CDP Lifecycle and Authentication Process}

In the most straightforward scenario, the digital template \t is printed using the industrial printer \( P_E \) to produce the physical CDP \x. This original CDP is then distributed to the public domain, and its image is captured by a device for authentication. The captured image is compared to the reference \r using a similarity metric \fsim. In the simplest approach, the reference is the digital template \t. However, this method is vulnerable to sophisticated attacks that can estimate and reproduce the digital template, creating convincing fakes.

To counter these sophisticated attacks, an advanced scenario involves estimating the digital template \th from the physical original CDP \x using a pre-trained model. This estimated template is then reprinted by the attacker printer \( P_A \) to produce the fake CDP \f. Both original and fake CDPs are distributed publicly, making it challenging to distinguish between them during probe acquisition.

A third approach, discussed in previous research (EUSIPCO 2024), involves enrolling the physical original CDP \x during the production stage by capturing and storing its image as \xe. This enrolled CDP is used as a reference to authenticate probes, significantly enhancing the similarity score when comparing identical physical objects. However, this method is costly and undermines the scalability and cost-efficiency of CDPs.

To address these limitations, we propose generating synthetic physical CDPs \xh from the digital template \t. This method requires only a small number of enrolled CDPs to train the model, which can then produce synthetic CDPs for authentication. Synthetic CDPs can serve as references, enabling robust and scalable authentication across various scenarios.

In summary, our authentication system evaluates the similarity between the probe \y and the reference \r using similarity metrics. These metrics are processed by a pre-trained classifier to determine the authenticity of the probe. By leveraging synthetic CDPs and advanced machine learning techniques, we aim to create a resilient and cost-effective authentication system capable of thwarting sophisticated attacks.

==> sections/04_results_old.tex <==
\section{Results}

\begin{figure*}
    \centering
    \begin{subfigure}{.49\textwidth}
        \includesvg[width=\textwidth]{figures/roc/HPI55_pcorr.svg}
        \caption{for HPI55}
        \label{fig:roc:55}
    \end{subfigure}
    \begin{subfigure}{.49\textwidth}
        \includesvg[width=\textwidth]{figures/roc/HPI76_pcorr.svg}
        \caption{for HPI76}
        \label{fig:roc:76}
    \end{subfigure}
    \caption{The ROC curves for $\fpcorr(\y, \r)$, where $\r \in \{\t, \xhat\}$ with a corresponding AUC value for every imaging system. $\xe$ isn't shown since its AUC equals 1.00 for all imaging systems.}
    \label{fig:roc}
    % \vspace{-4mm}
\end{figure*}

\input{sections/tables/aucs}


Referencing back to Fig. \ref{fig:scatter}, we have conducted only same-device experiments, meaning that the incoming probe $\y$ is compared to $\xe$ or $\xhat$ of the same physical and acquisitional origin. Nevertheless, the scenarios of cross-device testing should be performed in the future since certain pairs of imaging systems (like \textit{14 macro} and \textit{15 macro}) follow similar statistical distributions.

As expected from distributions shown in Fig. \ref{fig:scatter:scan} we obtain a similar degree of separability in $\fsim(\y, \t)$ cases for mobile phones. This is well-supported in Fig. \ref{fig:hist} (Digital $\t$ plots) and the trend is preserved for both printers. The indicated AUC value in plot's title is reflected in Fig. \ref{fig:roc} via respective ROC curve. A comprehensive comparison of $\fsim(\y, \t)$ performance for the full range of imaging systems is presented in Table \ref{tab:aucs}. The presented table allows to formulate the following important conclusions for $\fsim(\y, \t)$:

\begin{itemize}
    \item the separability rate increases with the imaging effective resolution;
    \item in certain cases the macro lenses drastically overpeform the scanner and are somewhat close to the ideal;
    \item overall mobile phone sampling yields a high degree of variability and uncertainty thus making AUC considerably fluctuate across imaging devices, but only for $\fsim(\y, \t)$;
    \item on average $\fssim$ renders itself less discriminative in contrast to $\fpcorr$;
    \item regardless of printer or imaging systems, neither combination provides a satisfactory AUC.
\end{itemize}

The next key point in our study is assessing the performance of $\fsim(\y, \xe)$. As shown in Fig. \ref{fig:hist} (Physical $\xe$ plots), even the oldest mobile phone in our study demonstrates negligible overlap between $\x$ and $\f$ for both printers, highlighting the superiority of the $\fsim(\y, \xe)$ approach. This trend is consistent across all acquisitions. When $\y = \x$, we effectively compute $\fsim(\x, \xe)$, where both $\x$ and $\xe$ originate from the same physical CDP, resulting in the highest possible mutual information. Consequently, $\fsim(\f, \xe)$ cannot achieve such a level of microstructural similarity. In Table \ref{tab:aucs} we observe the perfect separability for any pair of printer and imaging device. However, in the case of \textit{12 wide} AUC $\neq 1$ due to the alignment issues, which was discovered after manual investigation of the samples. Following these results we decided its unnecessary to include ROC curves for these results as they would not render themselves useful. To conclude:

\begin{itemize}
    \item the obtained results are well-aligned with a previous study\cite{chaban2024eusipco} and are explained by $\xe$ being a physically unclonable function (PUF) \cite{maes2013puf};
    \item $\fsim(\y, \xe)$ scenario sets an overwhemingly high bar for any potential authentication system, even possibly not achievable by other means and algorithms;
    \item employment of $\xe$ can be implemented in the applications, where no proposed authentication improvement can increase the classification accuracy;
    \item enrollment of $\xe$ may be expedient if the application is oriented for low-volume and low-end devices, such as iPhone XS.
\end{itemize}

Having two departing points covered above, we have the baselines for assessing the viability of synthetic $\xhat$, comparatively. The results shown in Fig. \ref{fig:hist} (Synthetic $\xhat$ plots) present the significant improvement in terms of AUC for $\fpcorr(\y, \xhat)$, when compared to $\fpcorr(\y, \t)$, regardless of printer. And as in previous scenarios, this tendency is preserved across all imaging devices as shown in Table \ref{tab:aucs} and in Fig. \ref{fig:roc}. In many scenarios $\xhat$ provides a perfect separabilty at AUC$=1$, though this may be due to a small sample size and with its increase AUC may decrease. The following list breaks down the main takeaways from the observed results:

\begin{itemize}
    \item $\xhat$ as reference $\r$ provides an enormous increase in separability between originals $\x$ and fakes $\f$;
    \item for scenarios where AUC$<1$ it is possible to implement a range of improvements like fine-tuning, data refinement and tweaks network architecture or loss function;
    \item though $\xhat$ still lags behind $\xe$ in terms of AUC, for certain imaging systems it is sufficient even in current implementation;
    \item AUC for scanner-based results is the lowest when compared to any mobile phone, highlighting the possibility that synthetic generator $S$ have learned the environmental conditions of $\xe$, which are more similar to $\x$ than for $\f$;
    \item a slightly better performance of $\fssim$ for HPI55/12 wide combination may be linked to generator $G$ loss function, which contains SSIM as a term, along with L2 and L1 norms.
\end{itemize}

Summarizing, the results have brought to light the separability of original $\x$ and fake $\f$ samples across various imaging systems, demonstrating that $\fpcorr(\y, \xhat)$ yields higher AUC values compared to $\fsim(\y, \t)$. Mobile phones show high variability in AUC, with macro lenses performing close to ideal in some cases. The $\fsim(\y, \xe)$ approach consistently achieves perfect separability due to the physically unclonable nature of $\xe$. The synthetic reference $\xhat$ enhances separability significantly, though still below $\xe$’s performance. Scanner-based results exhibit the lowest AUC, suggesting that the generator $S$ adapts better to mobile phone conditions. Overall, these findings underscore the potential for improved authentication using $\xe$ and $\xhat$ references, with implications for low-end device applications.

